Abundances of Baade's Window Giants from Keck/HIRES Spectra: II. The Alpha- and Light Odd Elements

We report detailed chemical abundance analysis of 27 RGB stars towards the Galactic bulge in Baade's Window for elements produced by massive stars: O, Na, Mg, Al, Si, Ca and Ti. All of these elements are overabundant in the bulge relative to the disk, especially Mg, indicating that the bulge is enhanced in Type~II supernova ejecta and most likely formed more rapidly than the disk. We attribute a rapid decline of [O/Fe] to metallicity-dependent yields of oxygen in massive stars, perhaps connected to the Wolf-Reyet phenomenon. he explosive nucleosynthesis alphas, Si, Ca and Ti, possess identical trends with [Fe/H], consistent with their putative common origin. We note that different behaviors of hydrostatic and explosive alpha elements can be seen in the stellar abundances of stars in Local Group dwarf galaxies. We also attribute the decline of Si,Ca and Ti relative to Mg, to metallicity- dependent yields for the explosive alpha elements from Type~II supernovae. The starkly smaller scatter of [<SiCaTi>/Fe] with [Fe/H] in the bulge, as compared to the halo, is consistent with expected efficient mixing for the bulge. The metal-poor bulge [<SiCaTi>/Fe] ratios are higher than ~80% of the halo. If the bulge formed from halo gas, the event occured before ~80% of the present-day halo was formed. The lack of overlap between the thick and thin disk composition with the bulge does not support the idea that the bulge was built by a thickening of the disk driven by the bar. The trend of [Al/Fe] is very sensitive to the chemical evolution environment. A comparison of the bulge, disk and Sgr dSph galaxy shows a range of ~0.7 dex in [Al/Fe] at a given [Fe/H], presumably due to a range of Type~II/Type~Ia supernova ratios in these systems.

==> tab4.tex <==
\clearpage
\LongTables
\begin{landscape}
\begin{deluxetable}{ccrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
%\tiny
%\rotate
\tablenum{4}
\tablewidth{0pt}
\tablecaption{Equivalent Width Measurements}
\tablehead{
\colhead{Wavelength} & \colhead{Ion} & \colhead{I-012} & \colhead{I-025} & \colhead{I-039} & \colhead{I-141} & \colhead{I-151} & \colhead{I-152} & \colhead{I-156} & \colhead{I-158} & \colhead{I-194} &  \colhead{I-202} & \colhead{I-264} & \colhead{I-322} & \colhead{II-033} & \colhead{II-119} & \colhead{II-122} & \colhead{II-154} & \colhead{II-172} & \colhead{III-152}  & \colhead{III-220} & \colhead{IV-003} & \colhead{IV-025} & \colhead{IV-047} & \colhead{IV-072} & \colhead{IV-167} & \colhead{IV-203} & \colhead{IV-325} & \colhead{IV-329} & \colhead{HR1184}& \colhead{HR1346} & \colhead{HR1348} & \colhead{HR1409} & \colhead{HR1411} & \colhead{HR1585} & \colhead{HR2035} & \colhead{HR2113} & \colhead{HR2443} & \colhead{HR3418} & \colhead{HR3733} & \colhead{HR3905} & \colhead{HR4104} & \colhead{HR4382} & \colhead{HR4450} & \colhead{HR4608} & \colhead{HR5340} \\
\colhead{\AA} & \colhead{} & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA} & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA} & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA} & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA} & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA} & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA} & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA} & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA}  & \colhead{m\AA} } 
\startdata
5577.34 & [O I] &  14 & \nodata &  26 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  11 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   9 &  13 &   9 & \nodata &   7 &  10 &  14 &  20 & \nodata &  18 &  15 & \nodata &  10 &   9 &  11 \\
6300.31 & [O I] &  71 &  48 &  60 &  56 &  60 &  61 &  44 &  63 &  60 & \nodata &  21 &  67 &  56 &  43 &  95 &  28 &  43 &  65 &  44 &  38 &  35 &  42 &  47 & \nodata &  52 &  32 &  54 &  26 &  25 &  38 &  27 &  22 &  42 &  33 &  59 &  45 &  41 &  17 &  50 &  61 &  35 &  21 & \nodata &  66 \\
6363.79 & [O I] &  33 &  22 &  31 &  32 &  26 &  22 &  20 &  28 &  22 &  19 &   8 &  29 &  25 &  13 &  66 &  12 &  18 &  21 &  25 &  17 &  11 & \nodata &  19 & \nodata &  23 & \nodata &  21 &  11 & \nodata &  13 &  10 & \nodata &  18 &  13 &  26 & \nodata & \nodata & \nodata &  20 &  24 &  14 & \nodata &  10 &  31 \\
5682.63 & Na I  & 130 & 208 & \nodata & 128 &  89 & 127 & 107 & 124 & 139 & 173 & 113 & 153 &  91 &  46 & 139 &  88 & 114 & 137 & \nodata &  45 & 121 & \nodata & 176 & 164 & 129 & \nodata & 101 & 100 & 140 & 123 & \nodata & \nodata & 129 &  95 & 116 & \nodata & \nodata & 104 & 212 & \nodata & 112 & 116 &  94 & 117 \\
5688.20 & Na I  & 156 & 236 & \nodata & 170 & 118 & 171 & 130 & 155 & 166 & 209 & 142 & 177 & 128 &  69 & 160 & 111 & 142 & 159 & 133 &  77 & 171 & 151 & 225 & 202 & 158 & \nodata & 122 & 119 & 166 & 144 & 169 & \nodata & 158 & 119 & 141 & \nodata & \nodata & 136 & 250 & \nodata & 141 & \nodata & \nodata & 148 \\
6154.23 & Na I  &  97 & 158 & 146 &  89 & \nodata &  98 &  55 &  78 &  98 & \nodata &  68 & 108 & \nodata & \nodata & \nodata &  33 &  74 &  91 &  60 & \nodata & \nodata & \nodata & 130 & \nodata & \nodata & \nodata &  46 &  43 &  99 &  76 &  97 &  96 &  75 &  39 &  69 &  84 & 130 &  54 & 152 & 110 &  65 &  78 &  45 &  74 \\
6160.75 & Na I  & \nodata & \nodata & 171 & \nodata & \nodata & \nodata & \nodata & \nodata & 112 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 150 & \nodata & \nodata & \nodata & \nodata &  58 & 105 &  90 & 118 & 111 &  97 &  64 &  92 & 101 & 141 &  72 & 173 & 125 &  78 &  98 &  70 &  95 \\
5711.09 & Mg I  & 162 & \nodata & \nodata & 155 & 117 & \nodata & 130 & 150 & 163 & \nodata & 128 & 155 & 129 &  96 & 136 & 122 & 141 & 156 & 134 &  94 & 158 & 161 & \nodata & \nodata & 126 & \nodata & 123 & 123 & 153 & 140 & 155 & 139 & 154 & 115 & 143 & 150 & 160 & 120 & 170 & 161 & 130 & 129 & 114 & 152 \\
6318.72 & Mg I  &  80 & 116 & 120 &  73 & \nodata &  81 &  57 &  70 &  84 &  80 &  41 &  72 &  58 &  22 & \nodata &  52 &  66 &  73 &  66 &  24 &  79 &  73 & 105 & 104 &  40 &  96 &  47 &  41 &  76 & \nodata &  75 & \nodata & \nodata &  45 &  64 & \nodata & \nodata &  44 &  84 & \nodata &  46 &  50 &  43 &  74 \\
6319.24 & Mg I  &  65 &  94 & 100 &  66 &  47 &  56 &  40 &  61 &  64 &  68 &  27 &  60 &  40 &  18 &  56 &  39 &  56 &  57 & \nodata &  17 &  56 &  66 &  86 &  92 &  25 &  88 &  40 &  30 & \nodata & \nodata &  53 & \nodata & \nodata &  35 &  55 & \nodata &  50 & \nodata &  65 & \nodata & \nodata & \nodata &  31 &  52 \\
6319.49 & Mg I  &  37 &  72 & \nodata &  37 &  21 &  33 &  19 &  38 &  42 &  42 &  14 &  35 &  20 & \nodata &  22 &  18 &  33 &  30 &  32 & \nodata &  32 &  35 &  57 &  65 &  11 &  60 &  10 &  15 & \nodata & \nodata &  25 & \nodata & \nodata &  15 &  27 & \nodata &  25 & \nodata &  40 & \nodata & \nodata & \nodata & \nodata &  31 \\
6765.45 & Mg I  & \nodata & \nodata & \nodata &  36 &  18 & \nodata & \nodata & \nodata &  42 & \nodata & \nodata &  29 &  21 & \nodata & \nodata & \nodata &  35 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  18 & \nodata &  21 &  32 &  25 & \nodata &  15 &  24 &  25 & \nodata & \nodata & \nodata &  21 &  16 & \nodata & \nodata &  25 \\
6799.00 & Mg I  &  43 &  93 &  88 &  44 &  24 &  52 & \nodata &  40 &  50 & \nodata &  14 &  42 &  24 & \nodata &  22 &  19 &  38 &  44 &  42 & \nodata &  44 &  39 &  71 & \nodata &  10 & \nodata &  18 &  27 &  45 &  30 &  45 &  36 &  34 &  23 &  30 &  38 &  44 &  24 &  61 &  30 & \nodata &  33 &  19 &  32 \\
6841.08 & Mg I  &  47 & 107 &  92 &  60 &  34 & \nodata &  31 &  54 & \nodata &  65 &  18 &  52 &  29 &  12 &  33 &  22 &  39 &  51 &  49 & \nodata &  56 &  42 & \nodata & \nodata &  16 &  93 &  23 &  28 & \nodata & \nodata & \nodata & \nodata & \nodata &  26 &  33 &  42 &  50 &  34 &  74 &  36 &  20 & \nodata &  24 &  37 \\
6894.92 & Mg I  & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  57 & \nodata & \nodata & \nodata & \nodata & \nodata &  33 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  82 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  31 & \nodata &  34 &  28 &  39 & \nodata &  44 \\
6965.41 & Mg I  &  60 & 128 & \nodata &  65 &  36 &  83 &  43 & \nodata & \nodata & \nodata &  26 &  59 &  43 & \nodata &  38 &  35 &  54 &  56 & \nodata &  14 &  88 &  52 & \nodata & 119 &  22 & 111 &  36 &  43 & \nodata &  51 &  70 & \nodata &  55 &  40 &  49 &  59 &  72 &  49 & \nodata &  44 & \nodata & \nodata &  38 &  55 \\
7387.69 & Mg I  &  94 & 147 & \nodata &  89 &  63 & 102 &  65 &  88 & \nodata & 100 &  46 &  92 &  66 &  38 & \nodata &  59 &  86 &  80 &  84 &  38 & 108 &  94 & \nodata & 148 &  37 & 131 &  62 &  73 &  95 &  70 & 103 &  86 &  81 &  62 &  75 &  87 &  94 &  76 & 116 &  68 &  65 &  85 &  55 &  81 \\
7875.43 & Mg I  & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  17 \\
5557.06 & Al I  &  42 &  93 &  98 &  39 &  18 &  54 &  18 &  47 & \nodata &  75 & \nodata &  57 &  23 & \nodata &  45 &  16 &  35 &  38 & \nodata & \nodata &  59 &  30 & \nodata &  79 & \nodata &  78 & \nodata &  18 &  41 &  26 &  42 &  28 &  26 &  14 &  30 &  37 &  42 &  12 &  73 & \nodata &  18 &  21 & \nodata &  25 \\
6696.02 & Al I  &  94 & 146 & \nodata & 104 &  66 &  96 &  63 &  97 & \nodata & 126 &  94 & 110 &  71 &  18 & 105 &  56 &  83 & 100 &  89 &  20 & 108 &  86 & \nodata & 142 &  71 & 146 &  57 &  61 &  93 &  83 &  95 &  83 &  81 &  59 &  87 &  82 & 118 &  52 & 132 & 110 &  56 &  69 &  50 &  84 \\
6696.79 & Al I  &  25 &  84 & \nodata &  34 &  12 &  43 &  13 &  33 & \nodata &  66 &  23 &  40 &  16 & \nodata & \nodata &  16 &  26 &  24 &  31 & \nodata &  56 & \nodata & \nodata &  68 & \nodata &  81 &   8 &  14 &  33 &  17 &  36 &  26 & \nodata &  12 &  20 &  22 &  38 &  14 &  63 &  31 &  12 &  21 &  11 &  17 \\
6698.67 & Al I  &  71 & 132 & \nodata &  71 &  38 &  64 &  36 &  77 & \nodata & 109 &  66 &  87 &  46 & \nodata &  74 &  32 &  61 &  72 &  58 &  10 &  89 &  55 & \nodata & 120 &  45 & 128 &  35 &  37 &  67 &  52 &  68 &  56 &  56 &  32 &  53 &  63 &  78 &  34 & 106 &  72 &  35 &  46 &  30 &  60 \\
7835.31 & Al I  & \nodata & \nodata & 136 & \nodata & \nodata & \nodata & \nodata & \nodata &  87 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 116 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  69 \\
7836.13 & Al I  & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  99 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 138 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  79 \\
5488.98 & Si I  &  31 &  50 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  27 & \nodata & \nodata &  27 &  23 & \nodata &  13 &  27 &  24 & \nodata & \nodata & \nodata & \nodata &  29 &  40 &  38 &  10 &  43 &  17 &  29 &  45 &  24 &  46 &  41 &  28 &  21 &  22 &  34 &  42 &  34 &  57 &  26 &  24 &  40 &  22 &  28 \\
5517.53 & Si I  & \nodata &  58 &  53 & \nodata &  27 & \nodata &  20 &  36 &  28 & \nodata &  14 &  33 &  26 & \nodata &  20 & \nodata &  29 &  26 & \nodata & \nodata &  37 & \nodata &  42 & \nodata & \nodata &  46 &  18 &  23 &  43 & \nodata &  42 & \nodata &  26 &  17 &  23 &  31 &  39 &  26 &  53 & \nodata &  21 &  32 &  20 &  22 \\
5701.10 & Si I  &  60 &  78 &  74 &  57 &  44 &  68 &  39 &  56 &  48 &  56 &  30 &  58 &  44 & \nodata &  32 &  47 &  51 &  49 & \nodata &  29 &  57 &  48 &  57 &  64 &  30 &  74 &  42 &  47 &  69 &  46 &  66 &  66 &  51 &  38 &  46 &  59 &  61 &  53 &  76 &  53 &  51 &  62 &  42 &  51 \\
6142.48 & Si I  &  40 &  59 &  56 &  41 &  26 &  43 &  26 &  34 &  35 &  48 &  20 &  40 &  30 &  15 &  18 & \nodata &  32 &  30 &  40 &  13 &  45 &  41 &  46 &  50 & \nodata &  57 &  26 &  40 &  51 &  36 &  58 &  58 &  35 &  30 &  32 &  44 &  50 &  44 &  56 &  31 &  30 &  46 &  35 &  33 \\
6145.02 & Si I  &  42 &  78 &  77 &  48 &  31 &  55 &  31 &  46 &  38 & \nodata &  22 &  44 &  29 & \nodata &  24 &  37 &  38 &  35 & \nodata &  17 &  52 &  36 &  55 &  69 &  19 &  66 &  29 &  44 &  58 &  40 &  61 &  59 &  42 &  35 &  35 &  47 &  53 &  45 &  65 &  37 &  41 &  52 &  34 &  38 \\
6155.13 & Si I  &  84 & \nodata & 115 & \nodata & \nodata &  85 &  65 &  78 &  68 & \nodata & \nodata & \nodata & \nodata &  43 & \nodata & \nodata & \nodata &  60 &  84 & \nodata & \nodata & \nodata &  90 & \nodata & \nodata & \nodata & \nodata &  74 & 106 &  73 & 110 & 108 &  88 &  65 &  68 &  88 &  97 &  92 & 120 &  71 &  68 &  97 &  74 &  73 \\
6635.69 & Si I  & \nodata & \nodata &  36 & \nodata & \nodata & \nodata & \nodata & \nodata &  12 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  20 &  26 & \nodata & \nodata & \nodata & \nodata &  28 &  14 &  25 &  26 &  18 & \nodata &  10 &  18 &  24 &  16 &  36 & \nodata &  12 &  17 & \nodata &  10 \\
7235.33 & Si I  &  42 & \nodata & \nodata & \nodata &  27 & \nodata & \nodata &  43 & \nodata &  39 &  24 & \nodata & \nodata & \nodata & \nodata & \nodata &  34 &  29 & \nodata & \nodata & \nodata &  36 & \nodata &  56 &  20 & \nodata & \nodata &  42 &  50 &  38 &  48 &  50 & \nodata &  29 & \nodata & \nodata &  48 & \nodata & \nodata & \nodata & \nodata & \nodata &  37 &  31 \\
7235.82 & Si I  &  30 &  46 & \nodata & \nodata & \nodata & \nodata & \nodata &  27 & \nodata &  32 & \nodata & \nodata &  18 & \nodata & \nodata &  23 &  26 &  20 & \nodata & \nodata & \nodata &  25 & \nodata &  36 & \nodata &  46 & \nodata &  28 &  34 & \nodata &  33 &  38 &  29 &  18 &  22 & \nodata & \nodata & \nodata &  51 & \nodata & \nodata & \nodata & \nodata &  20 \\
7250.63 & Si I  & \nodata &  80 & \nodata &  62 & \nodata &  65 &  40 &  52 & \nodata & \nodata &  34 &  59 &  42 &  31 & \nodata &  50 &  52 & \nodata & \nodata &  26 &  62 & \nodata & \nodata &  70 &  27 & \nodata &  44 & \nodata & \nodata &  48 &  87 &  81 &  41 & \nodata &  44 &  59 &  65 & \nodata &  75 & \nodata & \nodata &  69 &  52 &  58 \\
7423.50 & Si I  & \nodata & 130 & 133 & 101 &  85 & 113 & \nodata &  93 &  87 &  99 &  70 &  95 &  86 &  62 &  64 &  94 &  87 &  83 & 103 &  68 & 104 &  97 & 104 & 114 &  59 & 118 &  79 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  86 & \nodata & \nodata & 105 & 124 & \nodata &  88 & \nodata &  95 &  88 \\
7800.00 & Si I  & \nodata & \nodata &  74 & \nodata & \nodata & \nodata & \nodata & \nodata &  39 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  51 &  75 & \nodata &  63 &  65 & \nodata & \nodata & \nodata & \nodata & \nodata &  59 & \nodata & \nodata &  43 & \nodata & \nodata &  44 \\
5512.98 & Ca I  & 125 & 174 & \nodata & 134 & 103 & 128 & 100 & \nodata & 133 & 145 & 107 & 138 & 112 &  64 & 117 &  95 & 118 & \nodata & 123 &  70 & 121 & 118 & \nodata & \nodata & 115 & 146 & 102 & 101 & 130 & 110 & 122 & 121 & 119 &  92 & 116 & 128 & 145 & 106 & 149 & 140 & 107 & 105 &  90 & 118 \\
5590.11 & Ca I  & \nodata & \nodata & \nodata & 148 & 105 & \nodata & 114 & \nodata & 146 & 167 & 123 & \nodata & 127 &  88 & 141 & 100 & 120 & 146 & 135 &  94 & 137 & 134 & \nodata & \nodata & 143 & \nodata & 116 & 101 & 143 & 130 & 143 & 130 & 132 & 109 & 124 & 140 & \nodata & 110 & \nodata & \nodata & 121 & 113 & 106 & 139 \\
5867.56 & Ca I  &  72 & 112 & 102 &  68 &  38 & \nodata &  41 &  72 &  83 &  90 &  39 &  84 &  52 & \nodata &  59 &  39 &  62 &  65 &  69 &  18 & \nodata & \nodata &  95 & 109 &  46 &  92 &  42 &  38 &  60 &  52 &  69 &  67 &  64 &  38 &  51 &  64 &  78 &  39 &  87 &  78 &  45 & \nodata &  30 &  58 \\
6156.02 & Ca I  &  46 & \nodata &  76 & \nodata & \nodata &  51 &  25 &  51 &  55 & \nodata & \nodata & \nodata & \nodata &  10 & \nodata & \nodata & \nodata &  52 &  35 & \nodata & \nodata & \nodata &  76 & \nodata & \nodata & \nodata & \nodata &  19 & \nodata &  30 &  37 &  33 &  35 &  23 &  39 &  46 &  44 & \nodata &  64 &  64 &  26 & \nodata &  13 &  38 \\
6161.30 & Ca I  & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 118 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  79 & 111 & \nodata & 116 & 105 & \nodata &  85 & 107 & \nodata & \nodata &  87 & \nodata & \nodata &  89 &  96 &  69 & 107 \\
6166.44 & Ca I  & \nodata & \nodata & 156 & \nodata & \nodata & \nodata & \nodata & \nodata & 133 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  73 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  89 & 108 & 110 & 114 & 116 & 129 &  86 & 113 & 122 & 131 &  98 & 147 & 149 &  95 &  98 &  86 & 124 \\
6169.04 & Ca I  & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 163 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  90 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 110 & 133 & 140 & 147 & 134 & 143 & 109 & 135 & 143 & 168 & 118 & \nodata & \nodata & 127 & 127 & 110 & 145 \\
6455.60 & Ca I  & 119 & 166 & \nodata & 120 & \nodata & 119 & \nodata & 108 & \nodata & 141 & 100 & 137 & 103 &  48 & 126 &  75 & 101 & 111 &  98 &  59 & 119 & 105 & \nodata & 151 & 108 & 147 &  97 &  82 & 104 &  99 & 110 & 110 & 109 &  78 & 101 & 113 & 128 &  81 & 143 & 134 & \nodata &  88 &  72 & 110 \\
6471.66 & Ca I  & \nodata & \nodata & \nodata & 151 & 120 & \nodata & 126 & 143 & 161 & 173 & 140 & \nodata & 135 &  88 & 150 & 112 & 124 & 150 & 131 &  98 & 140 & 139 & \nodata & \nodata & 144 & \nodata & 131 & 118 & 143 & 140 & 152 & 148 & 144 & 112 & 138 & 149 & 161 & 117 & \nodata & \nodata & 127 & 121 & 108 & 146 \\
6499.65 & Ca I  & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 148 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & 110 & 135 & 134 & 140 & 131 & \nodata & 108 & 137 & 142 & \nodata & 113 & \nodata & \nodata & \nodata & 120 & 104 & 140 \\
6798.48 & Ca I  &  40 &  87 &  77 &  34 &  18 &  43 & \nodata &  40 &  48 & \nodata &  20 &  51 &  21 & \nodata &  41 &  19 &  34 &  45 & \nodata & \nodata &  37 &  28 &  72 &  74 &  16 &  60 &  12 &  13 &  30 &  21 &  30 &  27 &  32 &  14 &  25 &  28 &  44 &  12 &  61 &  46 & \nodata &  22 &  11 &  26 \\
7695.14 & Ca I  & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  20 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
5453.64 & Ti I  &  82 & 101 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  94 &  65 &  92 &  59 & \nodata & 102 &  21 &  60 & \nodata & \nodata &  16 & \nodata &  58 & \nodata & 105 &  75 & 116 &  58 & \nodata &  47 &  60 &  48 & \nodata &  72 &  31 &  76 &  60 &  73 &  24 &  88 &  90 &  38 &  31 &  19 &  77 \\
5618.35 & Ti I  &  28 &  40 &  48 &  28 & \nodata & \nodata & \nodata &  25 &  40 &  52 & \nodata &  33 & \nodata & \nodata &  39 & \nodata & \nodata &  33 & \nodata & \nodata & \nodata & \nodata &  58 &  47 &  18 &  44 &  12 & \nodata & \nodata & \nodata & \nodata & \nodata &  17 & \nodata &  20 &  16 &  17 & \nodata &  29 &  37 & \nodata & \nodata & \nodata &  17 \\
5648.56 & Ti I  & \nodata &  95 &  99 &  72 &  36 &  60 &  49 &  57 & \nodata &  86 &  51 &  79 &  52 &  19 &  85 &  26 &  56 &  74 &  62 &  15 &  74 &  56 &  95 &  96 &  57 &  93 &  50 &  35 &  38 &  60 &  53 &  44 &  57 &  32 &  68 &  64 &  67 &  34 &  82 &  85 &  37 &  45 &  26 &  63 \\
5739.47 & Ti I  &  77 &  96 &  90 &  73 &  38 &  63 &  46 &  65 & \nodata &  90 &  46 &  80 &  48 & \nodata &  87 &  22 &  50 &  72 &  59 &  14 &  57 &  56 &  90 &  89 &  55 &  93 &  43 &  28 &  42 &  48 &  49 &  38 &  54 &  28 &  62 &  56 &  62 &  27 &  79 &  79 &  36 & \nodata &  16 &  61 \\
5766.36 & Ti I  & \nodata & \nodata &  80 & \nodata & \nodata & \nodata & \nodata & \nodata &  58 & \nodata & \nodata & \nodata & \nodata & \nodata &  54 & \nodata &  38 & \nodata & \nodata &  10 &  54 & \nodata &  79 & \nodata & \nodata & \nodata &  20 &  25 &  37 &  39 &  34 &  32 &  40 &  24 &  42 &  43 &  55 &  22 &  69 &  61 &  22 &  32 &  19 &  42 \\
5913.73 & Ti I  &  63 &  72 & \nodata &  58 &  25 & \nodata & \nodata & \nodata & \nodata &  80 &  35 &  72 &  29 & \nodata & 108 &   8 &  29 &  65 & \nodata & \nodata &  34 & \nodata & \nodata &  74 &  69 &  72 &  26 & \nodata & \nodata &  28 &  12 & \nodata &  32 &   8 &  42 & \nodata &  31 & \nodata &  54 &  75 &  17 & \nodata & \nodata &  45 \\
5918.53 & Ti I  & 114 & 134 & \nodata & 115 &  78 &  94 &  81 & \nodata & \nodata & 128 &  98 & 128 &  94 &  40 & \nodata &  52 &  86 & 113 &  90 &  38 &  94 &  99 & \nodata & 130 & 125 & 139 &  94 &  57 &  70 &  94 &  78 &  68 & 110 &  60 & 108 &  98 & 108 &  53 & 122 & 143 &  71 & \nodata &  41 & 111 \\
5944.66 & Ti I  &  80 &  92 &  90 &  60 &  30 &  45 &  38 &  53 &  87 &  96 &  52 &  85 &  47 & \nodata & \nodata &  13 &  40 &  81 & \nodata & \nodata &  49 &  44 &  98 &  94 &  94 &  92 &  39 &  15 &  18 &  32 &  18 &  13 &  48 &  13 &  53 &  37 &  44 & \nodata &  66 &  93 &  18 & \nodata & \nodata &  66 \\
6092.79 & Ti I  &  71 &  88 &  87 &  66 &  30 &  45 &  36 &  52 &  75 &  81 &  39 &  75 &  44 & \nodata &  86 &  14 &  43 &  69 & \nodata &  10 &  57 &  42 &  90 &  88 &  46 &  83 &  39 & \nodata &  26 &  40 & \nodata & \nodata &  41 &  21 &  45 & \nodata & \nodata &  13 &  69 &  82 &  25 &  23 &  14 &  56 \\
6273.39 & Ti I  & \nodata & \nodata &  86 & \nodata & \nodata & \nodata & \nodata & \nodata &  65 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  77 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  19 & \nodata & \nodata & \nodata & \nodata &  35 & \nodata &  28 & \nodata &  52 &  69 &  11 & \nodata & \nodata &  40 \\
6706.29 & Ti I  &  14 &  27 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  32 & \nodata &  16 & \nodata & \nodata &  38 & \nodata & \nodata &  18 & \nodata & \nodata & \nodata & \nodata & \nodata &  31 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  12 & \nodata & \nodata & \nodata &  16 &  20 & \nodata & \nodata & \nodata & \nodata \\
6716.67 & Ti I  &  38 &  59 &  68 &  35 &  13 &  29 &  17 &  33 &  42 &  61 &  11 &  40 &  17 & \nodata &  59 &   7 &  21 &  36 & \nodata & \nodata &  35 &  18 &  66 &  64 &  23 &  54 &  18 & \nodata &  17 &  18 &  20 & \nodata &  19 &  11 &  23 &  22 &  33 & \nodata &  41 &  41 & \nodata &  13 & \nodata &  24 \\
6746.33 & Ti I  & \nodata & \nodata &  56 & \nodata & \nodata & \nodata & \nodata & \nodata &  37 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  59 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  17 &  14 &  24 & \nodata & \nodata &  33 & \nodata & \nodata & \nodata &  16 \\
7138.07 & Ti I  &  23 &  43 &  38 & \nodata & \nodata & \nodata & \nodata & \nodata &  36 &  45 & \nodata &  29 &  13 & \nodata & \nodata & \nodata & \nodata &  26 & \nodata & \nodata & \nodata & \nodata &  49 &  40 & \nodata &  30 &   8 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  19 &  12 &  17 & \nodata & \nodata &  34 & \nodata & \nodata & \nodata & \nodata \\
7271.51 & Ti I  &  75 & \nodata & \nodata &  65 &  35 &  52 &  32 &  56 &  78 & \nodata &  44 &  87 &  36 &  12 &  96 &  17 & \nodata & \nodata &  48 & \nodata & \nodata &  43 & \nodata & 106 &  57 & 102 &  34 & \nodata & \nodata &  38 & \nodata & \nodata & \nodata & \nodata &  55 &  47 &  64 &  12 & \nodata &  94 & \nodata &  21 & \nodata &  53 \\
7352.12 & Ti I  &  38 &  66 &  69 &  34 &  14 &  40 & \nodata &  33 &  42 &  58 &  14 &  40 &  23 & \nodata &  48 & \nodata &  21 &  40 & \nodata & \nodata &  40 & \nodata &  71 &  59 & \nodata &  60 &  18 & \nodata & \nodata &  17 & \nodata & \nodata &  23 & \nodata &  21 &  17 &  27 & \nodata &  47 & \nodata & \nodata & \nodata & \nodata &  28 \\
7391.51 & Ti I  &  28 &  50 & \nodata & \nodata & \nodata &  29 & \nodata &  21 & \nodata &  52 &  16 &  34 & \nodata & \nodata &  46 & \nodata &  14 &  27 & \nodata & \nodata & \nodata & \nodata & \nodata &  55 &  19 &  50 &  15 & \nodata & \nodata &  12 & \nodata & \nodata & \nodata & \nodata &  17 &  19 &  19 & \nodata &  28 &  48 & \nodata & \nodata & \nodata &  22 \\
7738.96 & Ti I  & \nodata &  34 &  40 & \nodata & \nodata & \nodata & \nodata & \nodata &  25 &  41 & \nodata &  17 & \nodata & \nodata & \nodata & \nodata & \nodata &  22 & \nodata & \nodata & \nodata & \nodata &  41 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  11 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  10 \\
5418.75 & Ti II & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  95 & \nodata &  88 &  76 & \nodata &  75 &  70 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  99 & \nodata &  88 &  86 &  79 &  88 &  84 &  93 &  76 & 102 &  96 &  98 &  78 &  99 & 107 &  91 &  83 &  78 &  98 \\
5492.86 & Ti II &  53 & \nodata &  74 & \nodata & \nodata & \nodata & \nodata & \nodata &  50 & \nodata & \nodata & \nodata & \nodata &  29 & \nodata & \nodata & \nodata & \nodata &  44 &  30 & \nodata & \nodata &  58 & \nodata & \nodata & \nodata & \nodata &  41 &  45 &  38 &  40 &  45 &  45 &  33 &  54 &  56 &  57 &  32 & \nodata &  60 &  40 &  44 &  34 &  49 \\
6606.95 & Ti II &  38 &  43 & \nodata &  33 & \nodata &  38 &  23 & \nodata &  31 &  44 &  29 &  38 &  30 &  20 & \nodata &  23 &  24 &  35 &  44 & \nodata &  30 &  36 &  47 &  43 &  27 &  40 &  28 &  29 & \nodata &  27 & \nodata & \nodata & \nodata &  21 & \nodata & \nodata & \nodata & \nodata &  33 & \nodata & \nodata & \nodata & \nodata &  34 \\
7214.72 & Ti II &  53 &  71 & \nodata &  62 &  46 &  68 &  43 &  39 &  51 &  61 &  45 &  63 &  48 &  38 &  68 &  46 &  40 &  41 & \nodata &  32 & \nodata &  55 & \nodata & \nodata &  45 &  70 &  42 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &  52 \\
\enddata
\end{deluxetable}
\end{landscape}

